Policy Distillation

Policies for complex visual tasks have been successfully learned with deep reinforcement learning, using an approach called deep Q-networks (DQN), but relatively large (task-specific) networks and extensive training are needed to achieve good performance. In this work, we present a novel method called policy distillation that can be used to extract the policy of a reinforcement learning agent and train a new network that performs at the expert level while being dramatically smaller and more efficient. Furthermore, the same method can be used to consolidate multiple task-specific policies into a single policy. We demonstrate these claims using the Atari domain and show that the multi-task distilled agent outperforms the single-task teachers as well as a jointly-trained DQN agent.

==> unused.tex <==
%!TEX root = policy_distillation.tex

\begin{table}[t]
\caption{Multi-Game Policy Distillation - Training and generalization mean scores on 10 Atari games.}
\label{sample-table}
\begin{center}
\scalebox{0.7}{
\begin{tabular}{lllllllllll}
\\ \hline \\
\multicolumn{1}{l}{\bf EVALUATION}  &\multicolumn{10}{c}{\bf RANDOM STARTS (USING NULL OPs, SAME AS TRAINING)} \\
\\ \hline \\
{\bf Agent}   & {\bf Beamrider}  & {\bf Breakout}   & {\bf Enduro}    & {\bf Freeway}   & {\bf Ms. Pac-Man}  & {\bf Pong}    & {\bf Q*bert}   & {\bf River Raid}   & {\bf Seaquest}  & {\bf Space Invaders} \\
\\ \hline \\
Teacher (DQN)  &9247.2  &349.9 &1040.7  &33.4  &3651.5  &19.3  &11633.0  &8556.8   &6045.4   &2081.9 \\
Dist-KL-4x   &8401.6  &412.5 &1018.3  &33.7  &3544.2  &19.6  &9925.5   &7130.8   &5297.8   &1845.7 \\
Multi-Dist-KL   &        &      &        &      &        &      &         &         &         & \\
\\ \hline \\
\multicolumn{1}{l}{\bf EVALUATION}  &\multicolumn{10}{c}{\bf HUMAN RANDOM STARTS (GENERALIZATION TESTING)} \\
\\ \hline \\
{\bf Agent}   & {\bf Beamrider}  & {\bf Breakout}   & {\bf Enduro}    & {\bf Freeway}   & {\bf Ms. Pac-Man}  & {\bf Pong}    & {\bf Q*bert}   & {\bf River Raid}   & {\bf Seaquest}  & {\bf Space Invaders} \\
\\ \hline \\
Teacher (DQN)  &9687.7  &384.9  &887.4   &28.1  &1106.3  &18.0  &9026.5  &5470.9  &4232.1  &1940.5 \\
Dist-KL-4x   &8854.3  &395.0  &891.5   &28.2  &857.7   &18.2  &7809.8  &4691.7  &4224.2  &1362.0 \\
Multi-Dist-KL  &5025.7  &256.1  &833.3   &27.8  &755.5   &17.6  &7968.3  &4676.9  &4449.5  &405.0 \\
\\ \hline \\
\end{tabular}
}
\end{center}
\end{table}



\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
%\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \includegraphics[width=8cm]{figures/comp_prev_work}
\end{center}
\caption{Comparison to previous work: performance relative to DQN.}
\end{figure}



\begin{table}[t]
\caption{Single-Game Policy Distillation - Mean Scores}
\label{sample-table}
\begin{center}
\scalebox{0.7}{
\begin{tabular}{lllllllllll}
\\ \hline \\
{\bf Agent}   & {\bf Beamrider}  & {\bf Breakout}   & {\bf Enduro}    & {\bf Pong}    & {\bf Q*bert}   & {\bf Seaquest}  & {\bf Space Invaders} \\
\\ \hline \\
UCT & 7233.0 & 406.0 & 788.0 & 21.0 & 18850.0 & 3257.0 & 2354.0 \\
Teacher (DQN) & 6845.9 & 401.2 & 301.8 & 18.9 & 10595.8 & 5286.0 & 1975.5 \\
Dist-KL-4x  & 7278.4 & 404.1 & 743.9 & 17.0 & 8963.5  & 4615.6 & 1862.0 \\
Dist-KL-15x   & 6176.9 & 386.9 & 777.3 & 17.7 & 9053.3  & 4729.6 & 1130.1 \\
Dist-KL-27x   & 6032.7 & 352.9 & 724.8 & 16.9 & 9377.3  & 3506.6 & 466.9  \\
UCC(-I)/UCR  & 5342.0 & 215.0 & 601.0 & 19.0 & 13189.0 & 2701.0 & 672.0  \\
\\ \hline \\
\end{tabular}
}
\end{center}
\end{table}



\begin{table}[t]
\caption{Multi-Game Policy Distillation - Training and generalization mean scores on 3 Atari games.}
\label{atari3_results_table}
\begin{center}
\scalebox{0.9}{
\begin{tabular}{lccc}
\\ \hline \\
\multicolumn{1}{l}{\bf EVALUATION}  &\multicolumn{3}{c}{\bf RANDOM STARTS} \\
\\ \hline \\
{\bf Agent}   & {\bf Freeway}   & {\bf Pong}    & {\bf Q*bert}  \\
\\ \hline \\
Multi-DQN       & 27.5 & 13.1 & 6060.8 \\
Multi-Dist-NLL  & 30.5 & 15.5 & 9340.8 \\
\\ \hline \\
\multicolumn{1}{l}{\bf EVALUATION}  &\multicolumn{3}{c}{\bf HUMAN RANDOM STARTS} \\
\\ \hline \\
{\bf Agent}   & {\bf Freeway}   & {\bf Pong}    & {\bf Q*bert}  \\
\\ \hline \\
Multi-DQN     & 23.3 & 12.0 & 3987.3 \\
Multi-Dist-NLL& 26.5 & 14.8 & 5678.0 \\
\\ \hline \\
\end{tabular}
}
\end{center}
\end{table}



\begin{table}[t]
\begin{center}
\caption{Comparison of distilled agents and
  DQN agents on 10 Atari games. The top table gives results when the games were
  initialized with a number of random moves. The bottom table gives
  results when the gameplay was started by a human player. }
\label{single_game_results_table}
\scalebox{0.7}{
\begin{tabular}{lcccccccccc}
\\ \hline \\
\multicolumn{1}{l}{\bf EVALUATION}  &\multicolumn{10}{c}{\bf RANDOM STARTS} \\
\\ \hline \\
{\bf Agent}   & {\bf Beamrider}  & {\bf Breakout}   & {\bf Enduro}    & {\bf Freeway}   & {\bf Ms. Pac-Man}  & {\bf Pong}    & {\bf Q*bert}   & {\bf River Raid}   & {\bf Seaquest}  & {\bf Space Invaders} \\
\\ \hline \\
Teacher (DQN) & 6845.9 & 401.2 & 301.8 & 30.3 & 2311.0 & 18.9 & 10595.8 & 8315.7 & 5286.0 & 1975.5 \\
Dist-KL-4x  & 7278.4 & 404.1 & 743.9 & 30.6 & 2278.7 & 17.0 & 8963.5  & 6960.7 & 4615.6 & 1862.0 \\
Dist-KL-15x   & 6176.9 & 386.9 & 777.3 & 30.6 & 2031.8 & 17.7 & 9053.3  & 6825.7 & 4729.6 & 1130.1 \\
Dist-KL-27x   & 6032.7 & 352.9 & 724.8 & 30.9 & 2093.7 & 16.9 & 9377.3  & 6106.7 & 3506.6 & 466.9  \\
\\ \hline \\
\multicolumn{1}{l}{\bf EVALUATION}  &\multicolumn{10}{c}{\bf HUMAN RANDOM STARTS} \\
 \\ \hline \\
{\bf Agent}   & {\bf Beamrider}  & {\bf Breakout}   & {\bf Enduro}    & {\bf Freeway}   & {\bf Ms. Pac-Man}  & {\bf Pong}    & {\bf Q*bert}   & {\bf River Raid}   & {\bf Seaquest}  & {\bf Space Invaders} \\
\\ \hline \\
Teacher (DQN)  & 8672.4 & 303.9  & 475.6 & 25.8 & 763.5 & 16.2 & 4589.8 & 4065.3 & 2793.3 & 1449.7 \\
Dist-KL-4x   & 7552.8 & 321.0  & 677.9 & 26.7 & 782.5 & 16.3 & 5947.3 & 4442.7 & 3986.6 & 1140.0 \\
Dist-KL-15x    & 7393.3 & 298.2  & 672.2 & 26.7 & 659.9 & 16.8 & 5994.0 & 4175.3 & 4567.1 & 716.1  \\
Dist-KL-27x    & 6521.2 & 238.8  & 556.7 & 26.7 & 734.3 & 15.7 & 4952.3 & 3417.9 & 3838.3 & 302.3  \\
\\ \hline \\
\end{tabular}
}
\end{center}
\end{table}

